LR-GLM: High-Dimensional Bayesian Inference Using Low-Rank Data Approximations

Due to the ease of modern data collection, applied statisticians often have access to a large set of covariates that they wish to relate to some observed outcome. Generalized linear models (GLMs) offer a particularly interpretable framework for such an analysis. In these high-dimensional problems, the number of covariates is often large relative to the number of observations, so we face non-trivial inferential uncertainty; a Bayesian approach allows coherent quantification of this uncertainty. Unfortunately, existing methods for Bayesian inference in GLMs require running times roughly cubic in parameter dimension, and so are limited to settings with at most tens of thousand parameters. We propose to reduce time and memory costs with a low-rank approximation of the data in an approach we call LR-GLM. When used with the Laplace approximation or Markov chain Monte Carlo, LR-GLM provides a full Bayesian posterior approximation and admits running times reduced by a full factor of the parameter dimension. We rigorously establish the quality of our approximation and show how the choice of rank allows a tunable computational-statistical trade-off. Experiments support our theory and demonstrate the efficacy of LR-GLM on real large-scale datasets.

==> conclusion.tex <==
% !TEX root =  submission.tex

We have shown through theory and experiments that low-rank data approximations can enable efficient, high-quality approximate posterior inference in large scale generalized linear models.
Our approximation is transparent; we provide interpretable error bounds for conjugate Gaussian regression as well as for Bayesian GLMs.
We demonstrate an attractive computational--statistical trade-off: increasing the rank of our approximation allows us to achieve higher quality approximations by investing more running time;
moreover, we recover the exact likelihood in the limit of a full rank approximation.
Lastly, we demonstrated that the error introduced by our approximation errs on the side of conservativeness; that is, we provide approximations that are never less uncertain than the exact posterior.
This conservativeness applies to both parameters and predictions.
We believe these properties of our low-rank data approximations make them a valuable and practical tool for approximate inference in large-scale Bayesian GLMs.

